Analytical Probability Distributions and EM-Learning for Deep Generative Networks

Deep Generative Networks (DGNs) with probabilistic modeling of their output and latent space are currently trained via Variational Autoencoders (VAEs). In the absence of a known analytical form for the posterior and likelihood expectation, VAEs resort to approximations, including (Amortized) Variational Inference (AVI) and Monte-Carlo (MC) sampling. We exploit the Continuous Piecewise Affine (CPA) property of modern DGNs to derive their posterior and marginal distributions as well as the latter's first moments. These findings enable us to derive an analytical Expectation-Maximization (EM) algorithm that enables gradient-free DGN learning. We demonstrate empirically that EM training of DGNs produces greater likelihood than VAE training. Our findings will guide the design of new VAE AVI that better approximate the true posterior and open avenues to apply standard statistical tools for model comparison, anomaly detection, and missing data imputation.

==> latent.tex <==




\subsection{Exact Computation of the Posterior}


\begin{thm}
It is NP-hard to obtain the exact posterior. It is NP-hard to compute the variational expectation.
\end{thm}

{\bf Test of the Monte-Carlo technique}.


\subsection{Deep Networks as Solvers}

Recall that in order to learn the parameters of the generator, one needs to infer the missing variables which are given by $\bz$. In a VAE, variational inference is done. Suppose we are given a distribution $q_{\bz|\bx,\gamma}$ which will guide the estimation procedure and also impact the {\em tightness} of the lower bound that EM maximizes. This tightness is given by the $KL$-divergence between $q_{\bz|\bx}$ and the true posterior $p_{\bz|\bx}$ as given by the Evidence Lower Bound (ELBO) derived below
\begin{align}
    \log(p_{\bx|\theta}(x))=\mathbb{E}_{q_{\bz|x,\gamma}}\left[\log \left( p_{\bx,\bz|\theta}(x,.)\right)\right]+H(q_{\bz|x,\gamma})+KL(q_{\bz|x,\gamma}||p_{\bz|x,\theta})
    \geq \mathbb{E}_{q_{\bz|x,\gamma}}\left[\log \left( p_{\bx,\bz|\theta}(x,.)\right)\right]+H(q_{\bz|x,\gamma}),\label{eq:ELBO}
\end{align}
which gives the Evidence Lower Bound (ELBO).
Then the Variational EM algorithm alternates between maximizing the tightness of the lower bound by finding the variational distribution that is the closest to the true posterior
\begin{align}
    \gamma^*=\argmax_{\gamma}\mathbb{E}_{q_{\bz|x,\gamma}}\left[\log \left( p_{\bx,\bz|\theta}(x,.)\right)\right]+H(q_{\bz|x,\gamma})
\end{align}
and then learning the generator weights based on this variational distribution as in
\begin{align}
    \theta^*=\argmax_{\gamma}\mathbb{E}_{q_{\bz|x,\gamma^*}}\left[\log \left( p_{\bx,\bz|\theta}(x,.)\right)\right]
\end{align}
In a VAE, $q_{\bz|x,\gamma^*}$ is given by a Gaussian with average and isotropic covariance matrix given by a DN, the encoder. This offers the following interesting result as a direct by product from the DN universal approximation property. First, by assuming some structure on the generator we can obtain the following result.

\begin{lemma}
The variational distribution given by a Gaussian with parameters given by a MASO DN corresponds to a mixture of truncated Gaussian.
\end{lemma}

\begin{thm}
The true posterior given a MASO encoder is a mixture of truncated Gaussian.
\end{thm}
\begin{proof}
The proof is direct since $p_{\bz|x,\Theta}\propto p_{\bx|\bz,\Theta}p_{\bz}$
\end{proof}


\begin{thm}
A DN parameterization of the variational inference will learn the true posterior in the limit of infinite width that is
\begin{align*}
    \min_{\gamma} \| q_{\bz|x,\gamma}-p_{\bz|x,\Theta}\|_2^2 \rightarrow_{K \rightarrow \infty} 0.
\end{align*}
\end{thm}

The above result is crucial. It serves as a guide justifying such technique. 


\subsection{Current Learning in DGNs}


Whenever $\mathbb{E}_{q_{\theta}(\bz|\bx)}\left[\log p_{\theta}(\bx,\bz)\right]$ can not be computed analytically, it is common to simply perform a Monte-Carlo sampling estimation. That is, sample a vector $\bz_i \sim q_{\theta}(\bz|\bx)$ and leverage the fact that 
\begin{align*}
    \mathbb{E}_{q_{\theta}(\bz|\bx)}\left[\log p_{\theta}(\bx,\bz)\right] \approx \frac{1}{N}\sum_{i=1}^N\log p_{\theta}(\bx,\bz_i) \;\;\text{ and }\;\;
    H(q_{\theta}(\bz|\bx)) \approx \frac{1}{N}\sum_{i=1}^N\log (q_{\theta}(\bz_i|\bx)),    
\end{align*}
where $\bz_i \sim q_{\theta}(\bz|\bx), i=1,\dots,N,$ and with the approximation becoming greater with $N$.


Given the ELBO bound, the EM algorithm simply performs a maximization-maximization procedure by first finding the optimal (per sample) variational parameters $\Theta_n$ and then leverage those to learn $\Theta$ by maximizing the likelihood with those estimates (notice that the Entropy term is independent of $\Theta$).





GLO is doing that \cite{celeux1992classification}











{\bf Partial E-step of VAEs:}

But then in a VAE you actually do not try to do the standard E step being
\begin{align*}
    \mu^*_n,\sigma^*_n=\argmax_{\mu,\sigma} ELBO(\mu,\sigma)
\end{align*}
but instead use a DN, called the {\em encoder} as a parametrization of those statistics and learn its parameters s.t.
\begin{align*}
    \mu(\bx_n),\sigma(\bx_n) \approx \argmax_{\mu,\sigma} ELBO(\mu,\sigma).
\end{align*}
That is, the encoder learns to solve a nonconvex optimization problem. Note that since $\bx_n$ are constant with the epochs and training iterations, the encoder simply needs to memorize the optimal settings for each point and simply adapt the evolution of $f_{\Theta}$ to adapt the optimum.

If the computation of the expectation was possible, the parameters of the variational distribution $q_{\theta}(\bz|\bx)$ would appear and backpropagation based learning could allow maximization of the ELBO. However due to the nonlinearity of $p_{\theta}(\bz,\bz)$, this computation is not tractable, cording the need to resort to sampling and estimation.
Estimation is done by sampling form the variational distribution as $\bz_i \sim \mathcal{N}(\mu(\bx),\sigma(\bx))$.  Doing better importance sampling has been done in \cite{burda2015importance} and showed better performances.

To do so, there is the need to apply thanks to the reparametrization trick, it is possible to sample $\bz_i \sim \mathcal{N}(0,I) \sigma(\bx)+\mu(\bx)$ allowing differentiability of the parameters $\mu(\bx)$ and $\sigma(\bx)$ while sampling from $\bz_i \sim \mathcal{N}(\mu(\bx),\sigma(\bx))$ would not allow backpropagation based learning of $\mu$ nor $\sigma$.

{\bf Partial M-step}
Thep artial M-step then simply optimizes the $\Theta$ parameters with gradient descent.






\subsection{Case Study: Gaussian Latent and Output Distribution}

\begin{figure}[!t]
\centering
\begin{minipage}{0.15\linewidth}
\centering
Implicit VAE \\
\begin{tikzpicture}[object/.style={thin,double,<->}]
\tikzstyle{main}=[circle, minimum size = 8mm, thick, draw =black!80, node distance = 7mm]
\tikzstyle{main2}=[circle, minimum size = 8mm, thick, draw =black!80, node distance = 7mm]
\tikzstyle{connect}=[-latex, thick]
\tikzstyle{box}=[rectangle, draw=black!100]
  \node[main] (s) [] {$Z$};
  \node[main2, fill = black!20] (x) [below=of s] { $X$};
  \path (s) edge [connect] (x);
%  \draw[dashed] (0.65,-2) -- (0.65,0.5);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.15\linewidth}
\centering
Explicit VAE\\
\begin{tikzpicture}[object/.style={thin,double,<->}]
\tikzstyle{main}=[circle, minimum size = 8mm, thick, draw =black!80, node distance = 7mm]
\tikzstyle{main2}=[circle, minimum size = 8mm, thick, draw =black!80, node distance = 7mm]
\tikzstyle{connect}=[-latex, thick]
\tikzstyle{box}=[rectangle, draw=black!100]
  \node[main] (t) [] {$T$};
  \node[main] (s) [below=of t] {$H$};
  \node[main2, fill = black!20] (x) [below=of s] { $X$};
  \path (t) edge [connect] (s)
        (s) edge [connect] (x);
%  \draw[dashed] (0.65,-2) -- (0.65,0.5);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.15\linewidth}
\centering
MPPCA/MFA\\
\begin{tikzpicture}[object/.style={thin,double,<->}]
\tikzstyle{main}=[circle, minimum size = 8mm, thick, draw =black!80, node distance = 7mm]
\tikzstyle{main2}=[circle, minimum size = 8mm, thick, draw =black!80, node distance = 3.3mm]
\tikzstyle{connect}=[-latex, thick]
\tikzstyle{box}=[rectangle, draw=black!100]
  \node[main2] (s) [] {$T$};
  \node[main2] (y) [left=of s] {$H$};
  \node[main, fill = black!20] (x) [below=of y] {$X$};
  \path (s) edge [connect] (x)
        (y) edge [connect] (x);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.5\linewidth}
\caption{
\small{(A) In a Gaussian mixture model (GMM), $[t]_1$ is a categorical variable that selects which of a number of Gaussian distributions is used to generate the observed input data $\bx$.
%
(B) In a factorial GMM (collaborative VQ model), each of the latent variables $[t]_d,\forall d$ contributes to forming the Gaussian from which $\bx$ is sampled. 
%
(C) In a mixture of principal components analysis (MPPCA) model, $[t]_1$ is a categorical variable that selects which of a number of linear subspaces is used to generate the observed input data $\bx$.
}}
\label{fig:PGMs}
\end{minipage}
\end{figure}

%\begin{tikzpicture}[object/.style={thin,double,<->}]
%\tikzstyle{main}=[circle, minimum size = 8mm, thick, draw =black!80, node distance = 7mm]
%\tikzstyle{main2}=[circle, minimum size = 8mm, thick, draw =black!80, node distance = 3.3mm]
%\tikzstyle{connect}=[-latex, thick]
%\tikzstyle{box}=[rectangle, draw=black!100]
%  \node[main2] (y) [] {$\bz$};
%  \node[main2] (s) [below right = 0.16cm and 0.6cm of y] {$\bt$};
%  \node[main, fill = black!20] (x) [below=of y] {$\bx$};
%  \path (s) edge [connect] (x)
%        (y) edge [connect] (s)
%        (y) edge [connect] (x);
%\end{tikzpicture}


\section{General Discrete Variable ELBO Derivation}


In our case we have an additional discrete random variable $\bt$. 
\begin{thm}
As long as the realizations of $\bt$ do not alter the nonlinearity states then the expectation can be computed as in a linear model case.
\end{thm}





Yet we make this random variable depend on $\bz$ as per the graphical model given in Fig.~\ref{}. With this formulation, the ELBO becomes
\begin{align*}
    \log(q_{\theta}(\bx))\geq & \mathbb{E}_{q_{\theta}(\bz,\bt|\bx)}\left[\log p_{\theta}(\bx,\bz,\bt)\right]+H(q_{\theta}(\bz,\bt|\bx))\\
    =  &\mathbb{E}_{q_{\theta}(\bt|\bx,\bz)q_{\theta}(\bz|\bx)}\left[\log p_{\theta}(\bx,\bz,\bt)\right]+H(q_{\theta}(\bt|\bx,\bz)q_{\theta}(\bz|\bx))\\
    =  &\mathbb{E}_{q_{\theta}(\bz|\bx)}\left[\mathbb{E}_{q_{\theta}(\bt|\bx,\bz)}\left[\log p_{\theta}(\bx,\bz,\bt)\right]\right]+H(q_{\theta}(\bt|\bx,\bz)q_{\theta}(\bz|\bx))&&\text{ (Fubini's Theorem)}\\
    \approx & \mathbb{E}_{q_{\theta}(\bt|\bx,\bz_i)}\left[\log p_{\theta}(\bx,\bz_i,\bt)\right]+H(q_{\theta}(\bt|\bx,\bz_i))-\log(q_{\theta}(\bz_i|\bx))&&\text{ (Monte-Carlo estimate of $\mathbb{E}_{q_{\theta}(\bz|\bx)}$)}
\end{align*}
with last line is the standard VAE approximation from a single sample approximation using $\bz_i \sim q_{\bz|\bx,\theta}$ and leveraging the reparameterization trick for differentiability. Now the key is that by leveraging the two following facts (i) $\bt$ being dependent on $\bz$ and the piecewise nonlinearity of $f_{\theta}$ we demonstrate that we compute the analytical form of () and thus have differentiable parameters for the discrete latent variable without resorting to any proxy and any other approximation.


Now the thing is that if it was not possible to analytically derive $\mathbb{E}_{q_{\theta}(\bt|\bx,\bz_i)}\left[\log p_{\theta}(\bx,\bz_i,\bt)\right]$ then we would have to resort to Monte-Carlo sampling as well, and due to the discrete nature of the random variable, there is not a reparameterization trick that would allow to gradient based learning of the parameters. Fortunately, we can make the DN activation function independent on the realization of $\bt$ and obtain the analytical form of this expression. 



\subsection{VAE Mixture and exact posterior}
VQ VAE somewhat ad hoc \cite{van2017neural}
DEC\cite{xie2016unsupervised} also somewhat ad hoc
then VADE \cite{jiang2016variational} with explicit GMM.
factorial \cite{paquet2018factorial}
trick of using GMM and with means that are one hot vectors !!!! \cite{pineau2018infocatvae}

needless to say that using categorical alone would be useless !


addition of an additional network to encoder this additional posterior density in GAN and VAE\cite{nalisnick2016stick,greff2017neural,zhao2018gan,yang2019deep,shi2019variational} or ad-hoc rules s.a. fixing the posterior as being uniform \cite{eghbal2019mixture}, or use Monte carle but can not learn the parameters \cite{dilokthanakul2016deep}. Flow based model are able to not resort to an additional DN \cite{liu2019neural}but impose very strict architecture of the GDN to be invertible, bijective, and thus $K=D$ and also impose architecture s.t. the inverse are fast to compute.




In the GMM vae you need the encoder to actually also predict the cluster probability directly and apply a softmax, here it is obtained directly from the expectation. The model is as follows.
The probabilistic graphical model is:
\begin{align*}
    \bz &\sim \mathcal{N}(0,\diag(\sigma^2_{z})),\\
    \bt &\sim Cat(\pi),\\
    \epsilon &\sim \mathcal{N}(0,\diag(\sigma^2_{x})),\\
    \bx &= f_{\theta}(\bz,\bt) + \epsilon,\\
    \bx|\bz=z,\bt=t &\sim \mathcal{N}(f_{\theta}(\bz,\bt),\diag(\sigma^2_{x}))
\end{align*}
the learnable parameters are $\theta, \sigma^2_{x}, \sigma^2_{z}$ and $\pi$.
and the nonlinear transformation is given by a standard DN with piecewise affine nonlinearities
\begin{align*}
    f_{\theta}(z,\bt)=\sum_{c=1}^C f^{(c)}_{\theta}(z)\Indic_{\bt=c}=&\sum_{c=1}^C\left(A^{(c)}_{L}(...(A^{(c)}_{1}z+B^{(c)}_{1})+\dots)+B^{(c)}_{L}\right)\Indic_{\bt=c}\\
    =&\sum_{c=1}^C\left( A^{(c)}_{L}\dots A^{(c)}_{1}z+\sum_{i=1}^{L}   A^{(c)}_{L} \dots A^{(c)}_{i+1}B^{(c)}_{i}\right)\Indic_{\bt=c}
\end{align*}
we can leverage our technique to derive the loss as follows
\begin{align*}
    \mathbb{E}_{p(\bt|x,z,\theta(t))}\left[\log( p(x|z,\bt,\theta))\right]=\mathbb{E}_{p(\bt|x,z,\theta(t))}\left[-\frac{1}{2\sigma^2}\|x-f_{\theta}(z,\bt) \|_2^2\right]
    =&\mathbb{E}_{p(\bt|x,z,\theta(t))}\left[-\frac{1}{2\sigma^2}\|x-\sum_{c=1}^C\Indic_{\bt=c}f^{(c)}_{\theta}(z) \|_2^2\right]\\
    =&\mathbb{E}_{p(\bt|x,z,\theta(t))}\left[-\sum_{c=1}^C\frac{\Indic_{\bt=c}}{2\sigma^2}\|x-f^{(c)}_{\theta}(z) \|_2^2\right]\\
    =-\sum_{c=1}^C\frac{1}{2\sigma^2}\|x&-f^{(c)}_{\theta}(z) \|_2^2\frac{[\pi(t)]_{c}\exp(-\frac{1}{2\sigma^2}\|x-f^{(c)}_{\theta(t)}(z) \|_2^2)}{\sum_{c=1}^C[\pi(t)]_{c}\exp(-\frac{1}{2\sigma^2}\|x-f^{(c)}_{\theta(t)}(z) \|_2^2)}
\end{align*}
\begin{align*}
    \mathbb{E}_{p(\bt|x,z,\theta(t))}\left[\log( p(\bt|\theta))\right]=\mathbb{E}_{p(\bt|x,z,\theta(t))}\left[\log(\prod_{c=1}^C[\pi]_c^{\Indic_{\bt=c}} )\right]    =&\mathbb{E}_{p(\bt|x,z,\theta(t))}\left[\sum_{c=1}^C\Indic_{\bt=c}\log([\pi]_c)\right]\\
    =&\sum_{c=1}^C\frac{[\pi(t)]_{c}\exp(-\frac{1}{2\sigma^2}\|x-f^{(c)}_{\theta(t)}(z) \|_2^2)}{\sum_{c=1}^C[\pi(t)]_{c}\exp(-\frac{1}{2\sigma^2}\|x-f^{(c)}_{\theta(t)}(z) \|_2^2)}\log([\pi]_c)
\end{align*}
this means that for the M step we have

\begin{align*}
T_{n,c}=&\frac{[\pi(t)]_{c}\exp(-\frac{1}{2\sigma^2}\|x_n-f^{(c)}_{\theta(t)}(z_n) \|_2^2)}{\sum_{c=1}^C[\pi(t)]_{c}\exp(-\frac{1}{2\sigma^2}\|x_n-f^{(c)}_{\theta(t)}(z_n) \|_2^2)}\\
    \pi^*=&\frac{1}{N}\sum_{n=1}^NT_{n,c}\\
    {\Sigma^{(c)}}^*=&\frac{\sum_{n=1}^NT_{n,c}(x_n-f^{(c)}_{\theta(t)}(z_n))(x_n-f^{(c)}_{\theta(t)}(z_n)^T}{\sum_{n=1}^N T_{n,c}}
\end{align*}

integrate the polytope polynomial
\url{https://math.nist.gov/mcsd/Seminars/2012/2012-09-19-DeLoera-presentation.pdf}
\url{https://arxiv.org/pdf/1908.06736.pdf}


it is NP-complete to find the smallest number of simplices for a polytope of dimension more than $3$ \cite{below2004computation}.
summary maybe \url{https://personales.unican.es/santosf/Talks/icm2006.pdf}

NP hard to do vertex enumeration problem for unbounded polytopes but very good otherwise \url{https://en.wikipedia.org/wiki/Vertex_enumeration_problem}
easy to integrate over a convex polytope in its V-representation \cite{lasserre1998integration}.
see \url{http://cgm.cs.mcgill.ca/~avis/doc/avis/AF92b.pdf}

\subsection{Measure of validity}
estimate the KL divergence between both distributions \url{https://www.princeton.edu/~kulkarni/Papers/Journals/j068_2009_WangKulVer_TransIT.pdf}
\subsection{A la Dropout}

We will derive 
$\log( p_{\theta}(\bx,\bz_i,\bt))=\log( p_{\theta}(\bx|\bz_i,\bt))+\log(p_{\theta}(\bt))+\log(p_{\theta}(\bz_i))$.
\begin{align*}
    f_{\theta}(\bz_i,\bt)=&T_{L}(A_{L}(...T_{1}(A_{1}\bz_i+B_{1})+\dots)+B_{L})\\
    =&T_{L}A_{L}\dots T_{1}A_{1}\bz_i+\sum_{i=1}^{L}   T_{L}A_{L}\dots T_{i+1}A_{i+1}B_{i} 
\end{align*}
with $T_{\ell}=\text{diag}(\bt_{\ell})$ and we also have that 
\begin{align*}
    \|T_{L}A_{L}\dots T_{1}A_{1}\bz_i \|_2^2=&\sum_{j=1}^D(\sum_{j_1,\dots,j_L}[T_{L}]_{j,j_{L}}[A_{L}]_{j_{L},j_{L-1}}\dots [T_{1}]_{j_1,j_0}[A_{1}\bz_i]_{j_0} )^2\\
    \| T_{L}A_{L}\dots T_{i+1}A_{i+1}B_{i} \|_2^2=&\sum_{j=1}^D(\sum_{j_i,\dots,j_L}[T_{L}]_{j,j_{L}}[A_{L}]_{j_{L},j_{L-1}}\dots [T_{i+1}]_{j_{i+1},j_i}[A_{i+1}B_i]_{j_i} )^2\\
    \langle T_{L}A_{L}\dots T_{i+1}A_{i+1}B_{i} ,T_{L}A_{L}\dots T_{i'+1}A_{i'+1}B_{i'}  \rangle =&\sum_{j}(\sum_{j_i,\dots,j_L}[T_{L}]_{j,j_{L}}[A_{L}]_{j_{L},j_{L-1}}\dots [T_{i+1}]_{j_{i+1},j_i}[A_{i+1}B_i]_{j_i} )\\
    & \times (\sum_{j_{i'},\dots,j_L}[T_{L}]_{j,j_{L}}[A_{L}]_{j_{L},j_{L-1}}\dots [T_{i'+1}]_{j_{i'+1},j_{i'}}[A_{i'+1}B_{i'}]_{j_{i'}} )\\
    \langle T_{L}A_{L}\dots T_{1}A_{1}\bz_i,T_{L}A_{L}\dots T_{i+1}A_{i+1}B_{i}  \rangle =& \sum_{j}(\sum_{j_1,\dots,j_L}[T_{L}]_{j,j_{L}}[A_{L}]_{j_{L},j_{L-1}}\dots [T_{1}]_{j_1,j_0}[A_{1}\bz_i]_{j_0} )\\
    & \times (\sum_{j_i,\dots,j_L}[T_{L}]_{j,j_{L}}[A_{L}]_{j_{L},j_{L-1}}\dots [T_{i+1}]_{j_{i+1},j_i}[A_{i+1}B_i]_{j_i} )
\end{align*}
\begin{align*}
    \|T_{L}(A_{L}(...T_{1}(A_{1}\bz_i+B_{1})+\dots)+B_{L})\|_2^2=&\|T_{L}A_{L}\dots T_{1}A_{1}\bz_i \|_2^2+\sum_{i=1}^{L}\| T_{L}A_{L}\dots T_{i+1}A_{i+1}B_{i} \|_2^2\\
    &+\sum_{ii'=1}^L\langle T_{L}A_{L}\dots T_{i+1}A_{i+1}B_{i} ,T_{L}A_{L}\dots T_{i'+1}A_{i'+1}B_{i'}  \rangle \\
    &+ \sum_{i=1}^{L}\langle T_{L}A_{L}\dots T_{1}A_{1}\bz_i,T_{L}A_{L}\dots T_{i+1}A_{i+1}B_{i}  \rangle 
\end{align*}

\begin{align*}
    \log( p_{\theta}(\bx|\bz_i,\bt))=&-\|\bx-f_{\theta}(\bz_i,\bt) \|_2^2\\
    =&\|\bx\|_2^2-2\langle \bx,f_{\theta}(\bz_i,\bt) \rangle+\| f_{\theta}(\bz_i,\bt) \|_2^2\\
    =&\|\bx\|_2^2-2\langle \bx,f_{\theta}(\bz_i,\bt) \rangle+\| f_{\theta}(\bz_i,\bt) \|_2^2
\end{align*}



\section{}








